Crank up the volume: preference bias amplification in collaborative recommendation

Recommender systems are personalized: we expect the results given to a particular user to reflect that user's preferences. Some researchers have studied the notion of calibration, how well recommendations match users' stated preferences, and bias disparity the extent to which mis-calibration affects different user groups. In this paper, we examine bias disparity over a range of different algorithms and for different item categories and demonstrate significant differences between model-based and memory-based algorithms.

==> FAT.tex <==
\section{Introduction}


%% Note: define research questions -- this is just the draft research questions, which is used for me to decide how to filter the original datasets for the experiments in our research; and also will be helpful for the following experiment design.

\begin{itemize}
    \item \textbf{RQ1} How do different recommendation algorithms propagate existing preference in the input data to the generated recommendation lists?
    %% Note: I just use the RQ1 used in the RMSE paper. this is still one of our goal, which will be achieved by involving a dataset from different domain and either validate or reverse the pattern in RMSE. 
    \item \textbf{RQ2} What factors do contribute to bias disparity and mis-calibration? 
    %%Note: this is the goal to find the reasons. In the experiments, it can be conducted from algorithm level (by comparing different algorithmic design choices) and from dataset level (by comparing the results from two dataset and find the consistent and inconsistent patterns between them)
\end{itemize}

\section{Related Work} % Nasim's 


\section{Methodology}
\subsection{Metrics} % Nicole's
% Reasons using two metrics -- providing insights from different perspectives
\subsubsection{Bias Disparity}
%% Note: in RMSE paper, the hidden assumption is that each category is exclusive, which means one movie is either Action or Romance, but the movie could not be both Action and Romance. In this paper, the metric is adjusted to solve this issue -- the solution is inspired by the approach taken in Steck's Calibrated Recommendations. (this part can be left as an add-on special condition explanation after the introduction of the metric)

% copy paste from Steck's, which is the inspiration how I will deal with the issue mentioned above. 
“Typically several genres g are assigned to a movie i in this data set–we assigned equal probabilities p(g|i) to each assigned genre g such that \sum{p(g|i)=1} for each movie i. ”

\subsubsection{Calibration Metric}

\subsection{Algorithms}
\subsection{Datasets} % Nicole's
We ran our experiments on two datasets from different domains, the MovieLens 1M\footnote{https://grouplens.org/datasets/movielens} dataset (ML) and the Yelp.com\footnote{https://www.yelp.com/dataset} dataset. 
% dataset's characteristics could be reasons for different patterns
% present essential information about datasets and related them with following discussion about experiment results
\subsubsection{MovieLens}
\subsubsection{Yelp.com}
In the original Yelp.com, it covers 6.7 million reviews from 1.6 million users on 192,609 businesses from different industries. 

In this research, we will only use the restaurant businesses. For each business, it does not have information presenting the type of business (e.g. restaurant, or gym). We combine information from business dataset, review dataset, and photo dataset to identify restaurants as many as possible. For example, in the business dataset, all the businesses including "RestaurantsTakeOut" as one of the attributes, or in the photo dataset, all the businesses including photos labeled as "food" are identified as restaurants. 

Out of computational consideration, we does not use all the metropolitan areas mentioned in the original Yelp dataset. We only select one city, Las Vegas, for experiment in this research. Shown in the Yelp dataset, Las Vegas is with the second most restaurants (after Toronto) but with most reviews among all the cities, far more than Toronto. Meanwhile, the users with more than 50 ratings of restaurant in Las Vegas are totally sufficient for this research. 

We use the business categories information (e.g. "Burger", "American (New)") in the business dataset as the way to present user's preference. The category amount of the resturants in Las Vegas could reach 565. In this research, we only use the region related labels (e.g. "American (New)", "Mexican") with no less than 50 restaurants using that label, leading to 18 categories selected for this research. Until now, the pre-process for the restaurant is ended with 3,994 restaurants from the 18 categories selected. 

% These selected categiries are 'American (Traditional)', 'Mexican', 'American (New)', 'Chinese', 'Italian', 'Japanese', 'Asian Fusion', 'Mediterranean', 'Hawaiian', 'Korean', 'Vietnamese', 'Tex-Mex', 'French', 'Latin American', 'Southern', 'Indian', 'Greek', 'Middle Eastern'.

Meanwhile, we only keep users with no less than 50 ratings over the selected restaurants, which leads to 760 users with 71,896 ratings. 

\subsection{Experiment Design}
% describe design based on the listed research questions 


\section{Experiment Results}
\subsection{Experiment 1: MovieLens}
\subsection{Experiment 2: Yelp.com}

\section{Conclusion and Future Work}

% Latent factors to categorize items and group users
In this paper and most researches \todo{include references}, the preference ratio is based on assigned categories, like Action or Romance genres in MovieLens, and American food or Mexican food categories in Yelp; and the discussion of group users mainly based on genetic or assigned group characteristics (e.g. male or female). In our future work, considering that these explicit labels on either items or users are the most obvious but definitely not the only way to categorize items or group users, we plan to extend the exploration to latent space.

==> body_v1.tex <==
\section{Introduction}
Recommender systems are ubiquitous, and they are influencing more and more on our daily decisions. Recently there has been a growing concern about the biases that exist in the results of recommender systems specially in contexts where fairness matters and is required by law such as credit (Equal Credit Opportunity Act), education (Civil Rights Act of 1964; Education Amendments of 1972), housing (Fair Housing Act), employment (Civil Rights Act of 1964) and etc. 

Take as a real-world example, the Amazon recruitment tool. It was designed to recommend a ranked list of qualified applicants to recruiters, but was shown to be discriminatory towards women and was shut down by the company itself in 2017 \cite{dastin2018amazon}. Also, XING\footnote{www.xing.com}, which is a job platform similar to LinkedIn, was found to rank less qualified male candidates higher than more qualified female candidates \cite{lahoti2019ifair}. 

Different kinds of biases might exist in the real world and they can be reflected in the training data and picked up, modeled and amplified by recommendation algorithms. This process can create and strengthen the filter bubbles wherein we live and can reinforce the stereotypes that can potentially lead to disparate impact.

In the recommendation field, a lot of metrics has been introduced to evaluate unfairness. Here in this paper, we have used bias disparity, a group-based metric based on \cite{tsintzou2018bias,zhao2017men}. This metric considers biases with respect to the preferences of specific user groups such as men or women towards specific item categories such as movie genres. This metric evaluates and compares the preference ratio (bias) in both the input and the output data and focuses on the role of recommendation algorithms in strengthening and weakening these biases.

Different classes of recommendation algorithms have various logic behind them and thus have different behaviors. \todo{extend}
In this paper, we analyze and compare the extent to which common collaborative filtering algorithms can change the existing biases. We have tested our experiments on a real-world dataset. We show how differently they reflect the bias in the results and as far as we know, this paper is among the first works to have observed this phenomenon in recommendation algorithms`. This analysis helps developers and researchers to beware of the discriminatory properties of CF algorithms and to think of removing the issues before designing a system.

We are interested in answering these questions: 
\begin{itemize}
    \item \textbf{How does bias change in the input dataset and the output recommendation?}
    \item \textbf{How does the bias change distribute among user groups? What factors drive the difference?}
    \item \textbf{One individual level question}
\end{itemize}
\todo{Roadmap}:talk about what will be presented in each section of the paper.

\section{Related work}
The biases seen in the outputs of recommendation algorithms can be due to many issues in the input data that we feed to the algorithms or as we say “garbage in, garbage out”. Among such potential causes \cite{barocas2016big} are sample size disparity, having limited features, proxy features, human factors, tainted examples and skewed findings. These causes are not mutually exclusive and can happen at the same time. 
Sometimes the data gathered on minority groups are so much less than the majority group that it becomes less likely to model the minority group perfectly (sample size disparity) or sometimes the important features for some sub-populations has so many missing values or unreliable values that it causes higher errors on these sub-populations (limited features). So the preferences of these users will be ignored by the model.
In some cases, even though the sensitive attributes (the attributes that shouldn't be considered in a task e.g. gender or race) are not included in the input data, there are some features that are proxies of sensitive attribute due to their correlation with them and will be creep into algorithms and will still cause the results to be biased.
Some entries in the data are tainted examples due to the biased decisions of humans. For example, in the case of Amazon recruitment tool, some decisions have been made before by previous managers which could have been biased. Then the model learning from this samples, replicates the human biases along with other information.
The biased samples can cause biased results. Having assumed that certain individuals are behaving in accordance with the biased sample can cause future mistreatment of those individuals and thus perpetuating the bias further and limiting the opportunity of certain groups in the society to prove the opposite trend. Here in this paper, we model the bias as the preference of users and their tendency to choose an item over the others. Although it is not a malicious bias, we are interested to see if this bias will be a cause of disparate impact similar to the others.
Applying machine learning algorithms blindly on the data, runs the risk of amplifying biases present in data. So we need to initially detect these biases and eventually control their influence by de-biasing the data, or mitigating their influence in the training process of the model or output results.
\todo{too much explanation about the causes of bias? paraphrase.}


Recently, there has been a shift of focus from achieving the best accuracy \cite{herlocker2004evaluating} in recommendations to beyond-accuracy measures such as diversity \cite{hurley2011novelty}, novelty and to more socially-sensitive fields such as fairness \todo{cite}.
As authors in \cite{burke2018balanced} mention, fairness can be a multi-sided notion. A recommendation system is a multi-sided setting \cite{burke2016towards} and fairness can be sought for different stakeholders that are involved such as item-providers, customers or the system. As an example, in a job recommender system, fairness for users/customers mean to provide similar recommendations to similar users without considering their demographic information. The offered methods that seek fairness for customers of a system fall under the category of customer-side fairness (C-fairness). XING scenario which was mentioned before, according to this definition is an example of unfairness for customers. 

The fairness for the item-providers/businesses, who look to hire candidates, means that both local businesses or startups and big corporations, have an equal chance of being exposed/recommended to good candidates. This kind of fairness is called the provider-side fairness (P-fairness). Fairness can be a part of a system goal besides utility, for example in this scenario, if the system tries to match the best job candidates who are a good fit for some companies while trying to meet the fairness needs of either or all the stakeholders. They system can have its own fairness goal as well, such as Kiva Funds\footnote{www.kiva.org}, a micro-lending crown-sourcing non-profit with the mission of providing equal access to capital for any loan-borrower worldwide.

To detect and model bias, several metrics have been introduced for recommendation problems. The metrics presented in \cite{yao2017beyond}, such as absolute unfairness, value unfairness, underestimation and overestimation unfairness focus on the discrepancies between the predicted scores and the true scores across protected and unprotected groups and consider the results to be unfair if the model consistently deviates (overestimates or underestimates) from the true ratings for specific groups. These metrics show unfairness towards customers.

Equality of opportunity discussed in \cite{hardt2016equality} cares about getting equal proportions of individuals from the qualified fractions of each group (equality in true positive rate). This metric can be used both to detect unfairness both for customers and providers.

\cite{celma2008hits} has discussed another type of bias called popularity bias. Many e-commerce websites have this kind of bias such that items from established sellers may dominate recommendation lists because they are more trusted due to having lots of reviews while newly-arrived sellers receive less attention. In this situation, the likelihood of being recommended for popular items will be considerably and unfairly higher than the rest of the items (long-tail items). The methods presented in \cite{abdollahpouri2017controlling, kamishima2014correcting} have tried to break the feedback loop and mitigate this issue. These methods generally try to increase fairness for item providers (P-fairness) in the system by diversifying the recommendation list of users.

There has been some work \cite{eskandanian2017clustering, liu2018personalizing} that try to increase fairness for item-providers by increasing a more diversified set of recommendations to users and some have also offered to consider user’s tolerance for diversity, or in other words users' preferences, to stay fair to customers as well.

Bias disparity paper \cite{tsintzou2018bias}, seeks to demonstrate unfairness for customers/users by modeling the bias as the preferences of users and here in this paper we are interested in tracking the change in user preference (user bias) that recommendation algorithms might have had one the results. The authors in \cite{channamsetty2017recommender} also looked into the influence of algorithms on the output data, but they tracked the change of diversity in user profiles in both the input and output data. \cite{ekstrand2018exploring} has also looked at the influence of collaborative algorithms on BookCrossing dataset when users tend to read books from males versus females. According to their results, both nearest neighbor methods and amtrix factorization propagate the biases and strengthen them.

\todo{to complete}

\section{Methodology}
\subsection{Bias Disparity Definition}
Let $\mathcal{U}$ be the set of $n$ users and $\mathcal{I}$ be the set of $m$ items and $S$ be the $n \times m$ input matrix, where $S(u,i) = 1$ if user $u$ has selected item $i$, and zero otherwise. 
 
Let $A_{U}$, be an attribute that is associated with users and partitions them into {\it groups} that have that attribute in common, such as gender. Similarly, let $A_{I}$ be the attribute that is associated with items and that partitions the items into {\it categories} sharing a similar attribute e.g. action or romance genres.
Given matrix $S$, the input {\it preference ratio} for user group G on item category C is the fraction of liked items by group $G$ in category $C$. Formula (1) is essentially the conditional probability of selecting an item from category C given that this selection is done by a user in group G.
\begin{equation}
    PR_{S}(G, C) = \frac{\sum_{u \in G}\sum_{i \in C} S(u, i)}{\sum_{u \in G}\sum_{i \in \mathcal{I}} S(u, i)} 
\end{equation}

Formula (1) is normalized by $P(C)$, where ${P(C) = {|C|}/{m}}$ is the probability of selecting from category C when we selecting uniformly at random. Then, {\it bias} $B_{S}(G, C)$ for group G on category C is defined as follows:

\begin{equation}
    B_{S}(G, C) = \frac{PR_{S} (G, C)}{P(C)}
\end{equation}

Then, {\it positive bias} or bias values greater than 1, happen when a group such as G, on average, tends to like an item category such as C more often. The opposite trend is true for {\it negative bias}.
To compute the bias change in the input $S$ and output of a recommendation algorithm $R$, {\it bias disparity}, that is the relative change of the bias value, is defined as follows:

\begin{equation}
    BD(G, C) = \frac{B_{R} (G, C) - B_{S}(G, C) }{B_{S}(G, C)}
\end{equation}

Assuming that a recommendation algorithm provides each user $u$ with a list of $r$ ranked items $R_{u}$, $R$ is the collection of all the recommendations to all the users represented as a binary matrix, where $R(u, i) = 1$ if item $i$ is recommended to user $u$, and zero otherwise.
For more details on this metric, interested readers can refer to \cite{tsintzou2018bias}.

In this paper, we use bias disparity metric on two levels: 1. for different user groups (e.g. women and men) to which we refer as {\it group-based} bias disparity or formula (3) and 2. for all the users in the dataset which we refer to it as {\it general} bias disparity or formula (4).

\begin{equation}
    BD(C) = \frac{B_{R} (C) - B_{S}(C) }{B_{S}(C)}
\end{equation}
\todo{Do we include formula 4?}

\subsection{Algorithms}
The focus of this research is about the collaborative filtering algorithmic bias. All the recommenders were built via the Librec-auto \cite{mansoury2018automating}, which is a wrapper built around the core LibRec \cite{guo2015librec} functionality. All the recommenders are built with user-fixed 5-fold cross validation. Multiple common used algorithms are selected for experiments, popularity based recommender, random based recommender, neighborhood based recommenders, and latent matrix factorization based recommenders. 

Popularity and random based recommenders serve as the baseline in this research. Popularity based recommender is about making recommendation based on the most rated items. Theoretically, popularity based algorithm is easy to transform the popularity bias to recommendation, which is the key reason why this is selected as a baseline algorithm for comparison. Random based recommender used in this research is the random guess, which random recommends the items among all available items. Theoretically, the population of different item categories plays important role in the bias disparity of the recommender. This provides a different baseline perspective from popularity based algorithm. 

The two primary areas in collaborative filtering are neighborhood-based and latent factor model based methods \cite{koren2009matrix}. These two areas are the main areas for experiments in this research. For the neighborhood methods, both user-based and item-based are experimented in this research. For latent factor model based collaborative filtering, Biased Matrix Factorization (BiasedMF)\cite{paterek2007improving}, Bayesian Probabilistic Matrix Factorization (BPMF)\cite{salakhutdinov2008bayesian}, and Weighted Regularized Matrix Factorization (WRMF)\cite{hu2008collaborative}, are used for experiments. 

\subsection{Datasets}

The dataset mainly used in this research is the MovieLens 1M \footnote{https://grouplens.org/datasets/movielens} (ML), a publicly available dataset for movie recommendation which is widely used in Recommender system's domain. ML contains 6,040 users and 3,702 movies and 1M ratings. Sparsity of ratings in this dataset is about 96\%. 

In this paper, we executed two sets of experiments, respectively with Action and Romance movies, and with Crime and Sci-Fi movies. The original ML dataset is filtered based on design of different experiments. The two sets of genres present different prototypes. Both sets have biased input preference but with different sources. The preference bias in the Action and Romance pair comes from the male group, while the female group has a balanced preference over the two genres. The preference bias in the Crime and Sci-Fi comes consistently from both group, which means the preference ratios of the two genres for the two user groups are similar. The comparison of the two experiment sets can present how the bias disparity change for the whole population and sub groups with different bias sources. \todo{add table describing the characteristics of the two datasets}



\subsection{Experiment Design}

For both experiment sets, the experiment design is similar. First part of the experiment is based on the whole population. Results from this part can present whether the recommendation is with algorithmic bias. If the input preference ratio is significantly different from the output preference ratio in the recommendation, or say the bias disparity is significant different from 0, it proves the existence of algorithmic bias. 

The second part is based on grouped bias disparity. In this part, the bias disparity is calculated based on the group bias change using the original bias disparity metric in \cite{tsintzou2018bias}, which presents how the bias change of the whole population distributes between groups. If the bias disparity changes to the same degree for different user groups, it shows the algorithm comes with bias but it's fair for different groups. Otherwise, the recommender comes with not only algorithmic bias but also unfairness issue. 

About the fairness discussion, it can be divided into two levels. The first level is without the consideration of the context. For discussion at this level, it is fair if the values of bias disparity of two groups are similar. Otherwise, the recommendation introduces uneven influence on two user groups, which is defined as unfairness. The second level is about the fairness discussion including context, which is mainly based on the prior condition, the input preference ratio. The input preference ratio presents the initial group preference. If the output preference is kept the same or amplified for the group, it's the fair situation for the group. Otherwise, it's unfair for the group because their preference is not well presented in the recommendation. 

\todo{diagram?}

\section{Results}
\subsection{Experiment One: Action and Romance}
In this experiment, the Action and Romance genres are taken as item categories, with 468 and 436 movies in each group respectively; meanwhile, users with over 90 ratings on Romance and Action movies are selected, resulting in 278 female and 981 male users. After the filtering, we ended up with 207,002 ratings from 1,259 users are used for experiment one. Based on the preference ratios of the whole population and sub groups shown in Table \ref{ar_input_pref}, the whole population prefer Action movies to Romance, which bias mainly comes from the biased preference from the male user group. 

\begin{table}[!hbtp]
\centering
\caption{Input Preference Ratio for Action and Romance}
\label{ar_input_pref}
\begin{tabular}{llll}
\hline
\textbf{Genre}  & \vline \textbf{Whole Population} & \vline \textbf{Male}  & \vline \textbf{Female} \\ \hline
Action     & \vline  0.675 & \vline  0.721 & \vline  0.502 \\ \hline
Romance     & \vline  0.325 & \vline  0.279 & \vline  0.498   \\ \hline
\end{tabular}
\end{table}

\subsubsection{Whole Population}

In Figure \ref{fig:ac_pr_all}, the bar shows the preference ratio in the recommendation output and the dashed line shows the input preference ratio for related categories. 

For Action category, it's the more preferred one between the two categories (0.678). The two neighborhood methods, UserKNN and ItemKNN, both significantly increase the preference ratio. The latent factor model based algorithms, Biased Matrix Factorization (BiasedMF), Bayesian Probabilistic Matrix Factorization (BPMF)\cite{salakhutdinov2008bayesian}, and Weighted Regularized Matrix Factorization (WRMF)\cite{hu2008collaborative}, shows different effect on the preference. None of the matrix factorization algorithms significantly increase the original input preference ratio. For BiasedMF, it significantly decreases the preference ratio in the recommendation, while for BPMF and WRMF, the output preference ratio is very close to the input preference ratio value. 

For Romance category, it has lower input preference ratio, which means in the input dataset, the overall population prefer Action to Romance. As a less favorable category, the preference ratios of Romance show a pattern reverse to the more favorable category, Action. The neighborhood algorithms decrease the preference ratio and the matrix factorization algorithms don't decrease the preference ratio. For biased matrix factorization, it increases the preference ratio, while for the other two matrix factorization algorithms, they don't change the preference ratio very significantly. 

The bias disparity showing in Figure \ref{fig:ac_bd_all} presents the percentage-wise changes of the preference ratio of the two categories over multiple algorithms, which are consistent with the observations from Figure \ref{fig:ac_pr_all}.\todo{extend}

\todo{better viz}
\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_pr_all.png}
    \caption{Post Preference Ratio for Action and Romance}
    \Description{Post preference ratio for the action and romance movie, this is for the whole population and unbalanced dataset}
    \label{fig:ac_pr_all}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_bd_all.png}
    \caption{Bias Disparity for Action and Romance}
    \Description{Bias disparity for the action and romance movie, this is for the whole population and unbalanced dataset}
    \label{fig:ac_bd_all}
\end{figure}

\subsubsection{Grouped Population}

For item category Action, for both male and female user groups, the neighborhood methods, UserKNN and ItemKNN, can drive up the preference ratio. The preference changes based on the matrix factorization algorithms are not totally consistent for the two groups except the BiasedMF. With BiasedMF, the preference ratio is lower than the input preference for both groups; with BPMF, the preference ratio of the female group is lower than the input preference ratio, while the male group has a very close preference ratio to the input; with WRMF, the inconsistency is more obvious -- the female group has lower preference ratio and male group is with higher preference ratio. 

For item category Romance, the phenomenon is similar with the reverse version of Action. For both groups, the neighborhood methods can lower the preference ratio. Different from category Action, the absolute value of the bias disparity for the two user groups are not similar. The male group is with higher absolute value of the bias parity. About the matrix factorization based algorithms, the preference changes are still inconsistent. With BiasedMF, the preference ratio is higher than the input preference ratio for both groups; with BPMF, the female group has a higher preference ratio, while the male group has similar prefernce ratio as input; with WRMF, the female group has higher preference and male group has lower preference. 

Based on the phenomenon from the two groups over multiple algorithms, some consistent patterns show the characteristics of algorithms. The neighborhood methods provides consistent bias disparity for both user groups. 

The bias disparity over different groups and categories is helpful when looking into the fairness issue. It shows how much the recommendation is different from the group's original preference. 

From the first level fairness perspective, ItemKNN introduces more bias to female group than male group in both category Action and Romance, while UserKNN provides more bias to male group than female group in both categories. For BiasedMF, it brings more bias to male group; for BPMF, it brings more bias to female group; for WRMF, the bias disparity shows different direction for male and female groups. When just comparing the absolute value of the bias disparity, for WRMF, it brings more bias to female group than male group. 

From the second level fairness perspective, female group has an almost balanced preference over Action and Romance movies, while male group prefers Action movies to Romance movies. In this case, only balanced preference in the recommendation is fair for female group. However, with the influence of the male group, none of the recommender algorithms provides fairness to the female group. For male group, the neighborhood methods and WRMF amplify the bias and BPMF keep the bias consistent with the input bias, which can be considered as a fair recommendation for male group. Among all the algorithms, BiasedMF is the only one that significantly dampens the bias for male group, which can be considered as a not fair recommendation because it recommends items against the initial preference. 

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_pr_grouped.png}
    \caption{Post Preference Ratio for Action and Romance of Different User Groups}
    \Description{Post preference ratio for the action and romance movie, this is for the grouped population and unbalanced dataset}
    \label{fig:ac_pr_grouped}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_bd_grouped.png}
    \caption{Bias Disparity for Action and Romance of Different User Groups}
    \Description{Bias disparity for the action and romance movie, this is for the grouped population and unbalanced dataset}
    \label{fig:ac_bd_grouped}
\end{figure}

\begin{table}[!hbtp]
\centering
\caption{First Level Fairness for Action and Romance}
\label{ar_first_fairness}
\begin{tabular}{ll}
\hline
\textbf{Algorithm}  & \vline \textbf{More biased group}   \\ \hline
ItemKNN     & \vline  Female \\ \hline
UserKNN     & \vline  Male    \\ \hline
BiasedMF    & \vline  Male  \\ \hline
BPMF        & \vline  Female  \\ \hline
WRMF        & \vline  Male \\ \hline
\end{tabular}
\end{table}

\subsection{Experiment Two: Crime and Sci-Fi}
The other experiment is based on the two genres, Crime and Sci-Fi, respectively with 211 and 276 movies. Users with over 50 ratings of movies from the two genres are selected and are used for the following experiment, resulting 259 female users and 1,335 male users. It turns out to be the experiment dataset including 37,897 ratings from the 1,594 users. Based on preference shown in Table \ref{cs_input_pref}, the whole population prefer Sci-Fi movies to Crime movies, and for two sub user groups, they have similar preference as the whole population. 

\begin{table}[!hbtp]
\centering
\caption{Input Preference Ratio for Crime and Sci-Fi}
\label{cs_input_pref}
\begin{tabular}{llll}
\hline
\textbf{Genre}  & \vline \textbf{Whole Population} & \vline \textbf{Male}  & \vline \textbf{Female} \\ \hline
Crime     & \vline  0.317 & \vline  0.302 & \vline  0.334 \\ \hline
Sci-Fi     & \vline  0.683 & \vline  0.698 & \vline  0.666   \\ \hline
\end{tabular}
\end{table}

\subsubsection{Whole Population}
As shown in the Figure \ref{fig:cs_pr_all}, the pattern of Crime and Sci-Fi over the whole population is consistent with Action and Romance. The neighborhood based algorithms, UserKNN and ItemKNN, increase the preference of category with the higher input preference, meanwhile decrease the preference of less favorable category. The matrix factorization based algorithms show different patterns from neighborhood based algorithms but very similar pattern as it's shown in the experiments with Action and Romance. For BiasedMF, it has the most significant effects on preference, which increase the preference of less favorable category and decrease the prefernce of the more favorable category. For BPMF and WRMF, the preference change is not that obvious. 

The bias disparity showing in Figure \ref{fig:cs_bd_all} presents the percentage-wise changes, which is also consistent with the bias disparity shown in the Figure \ref{fig:ac_pr_all} of experiment one.

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_pr_all.png}
    \caption{Post Preference Ratio for Crime and Sci-Fi}
    \Description{Post preference ratio for the Crime and Sci-Fi movie, this is for the whole population and unbalanced dataset}
    \label{fig:cs_pr_all}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_bd_all.png}
    \caption{Bias Disparity for Crime and Sci-Fi}
    \Description{Bias disparity for the Crime and Sci-Fi movie, this is for the whole population and unbalanced dataset}
    \label{fig:cs_bd_all}
\end{figure}

\subsubsection{Grouped Population}
Overall, the bias disparity of the grouped population patterns is very similar to the whole population pattern. Based on patterns shown in Figure \ref{fig:cs_pr_grouped}, the difference between two groups of same category and algorithm is small. 

From the first level fairness perspective, the difference of bias disparity's absolute value between groups is not as enormous as the difference shown in Action and Romance (Figure \ref{fig:ac_bd_grouped}), which is partly because the two groups have similar preference over Crime (0.3) and Sci-Fi (0.7). 

From the second level fairness perspective, neighborhood based algorithms can amplify the existing preference bias for both groups. The matrix factorization based algorithms either dampen the input preference ratio, like BiasedMF and BPMF, or don't significantly change the input preference, like WRMF. 


\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_pr_grouped.png}
    \caption{Post Preference Ratio for Crime and Sci-Fi of Different User Groups}
    \Description{Post preference ratio for the Crime and Sci-Fi, this is for the grouped population and unbalanced dataset}
    \label{fig:cs_pr_grouped}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_bd_grouped.png}
    \caption{Bias Disparity for Crime and Sci-Fi of Different User Groups}
    \Description{Bias disparity for the Crime and Sci-Fi movie, this is for the grouped population and unbalanced dataset}
    \label{fig:cs_bd_grouped}
\end{figure}

\begin{table}[!hbtp]
\centering
\caption{First Level Fairness for Crime and Sci-Fi}
\label{ar_first_fairness}
\begin{tabular}{ll}
\hline
\textbf{Algorithm}  & \vline \textbf{More biased group}   \\ \hline
ItemKNN     & \vline Female \\ \hline
UserKNN     & \vline Female    \\ \hline
BiasedMF    & \vline Male \\ \hline
BPMF        & \vline Male  \\ \hline
WRMF        & \vline Male(f=10) and Female(f=20)  \\ \hline
\end{tabular}
\end{table}

\section{Discussion}
When there’s an existing general bias in the data, some of the recommendation algorithms, such as K nearest neighbor method, perpetuate these biases whereas some other methods like matrix factorization reverses the bias. As we have discovered in our experiments, recommendation algorithms don’t explicitly benefit or harm specific user groups (in our case men and women) or item groups (genres), but they pick up a bias in the data that might be in favor or against a group and change them.\todo{to extend}


==> body_v2.tex <==
\section{Introduction}
Recommender systems are ubiquitous, and they are influencing more and more on our daily decisions. Recently, there has been a shift of focus from achieving the best accuracy \cite{herlocker2004evaluating} in recommendations to beyond-accuracy measures such as diversity, novelty and to more socially-sensitive fields such as fairness \cite{hurley2011novelty, jannach2015recommenders}. The main concern is about the biases that exist in the results of recommender systems specially in contexts where fairness matters and is required by law such as credit (Equal Credit Opportunity Act), education (Civil Rights Act of 1964; Education Amendments of 1972), housing (Fair Housing Act), employment (Civil Rights Act of 1964) and etc. 

Take as a real-world example, the Amazon recruitment tool. It was designed to recommend a ranked list of qualified applicants to recruiters, but was shown to be discriminatory towards women and was shut down by the company itself in 2017 \cite{dastin2018amazon}. Also, XING\footnote{www.xing.com}, which is a job platform similar to LinkedIn, was found to rank less qualified male candidates higher than more qualified female candidates \cite{lahoti2019ifair}. 

The biases seen in the outputs of recommendation algorithms can be due to many issues in the input data that we feed to the algorithms or as the saying goes: “garbage in, garbage out”. Among such potential causes \cite{barocas2016big} are sample size disparity, having limited features on minority groups, features that are proxies of demographic attributes, human factors or skewed findings. These causes are not mutually exclusive and can happen at the same time. Here in this paper, we model the bias as the preference of users and their tendency to choose an item over the other. 
These kinds of biases has helped recommendation algorithms to detect common patterns and provide users with personalized outputs. We know that these kinds of biases can cause filter bubbles \cite{pariser2011filter} and we are interested to see how the algorithms might change these biases and if they can be a cause of disparate impact similar to the others.

In the recommendation field, a lot of metrics has been introduced to evaluate unfairness. Here in this paper, we have used bias disparity, a group-based metric based on \cite{tsintzou2018bias,zhao2017men}. This metric considers biases with respect to the preferences of specific user groups such as men or women towards specific item categories such as movie genres. This metric evaluates and compares the preference ratio (bias) in both the input and the output data and focuses on the role of recommendation algorithms in strengthening and weakening these biases.

Different classes of recommendation algorithms have various logic behind them and thus have different behaviors. \todo{extend}
In this paper, we analyze and compare the extent to which common collaborative filtering algorithms can change the existing biases. We have tested our experiments on a real-world dataset. We show how differently they reflect the bias in the results and as far as we know, this paper is among the first works to have observed this phenomenon in recommendation algorithms`. This analysis helps developers and researchers to beware of the discriminatory properties of CF algorithms and to think of removing the issues before designing a system.

We are interested in answering these questions: 
\begin{itemize}
    \item \textbf{RQ1} How does bias change in the input dataset and the output recommendation?
    \item \textbf{RQ2} How does the bias change distribute among user groups?
    \item \textbf{RQ3} One individual level question \todo{extend}
\end{itemize}
\todo{Roadmap}:talk about what will be presented in each section of the paper.

\section{Related work}
As authors in \cite{burke2018balanced} mention, fairness can be a multi-sided notion. A recommendation system is a multi-sided setting \cite{burke2016towards} and fairness can be sought for different stakeholders that are involved such as item-providers, customers or the system. As an example, in a job recommender system, fairness for users/customers mean to provide similar recommendations to similar users without considering their demographic information. The offered methods that seek fairness for customers of a system fall under the category of customer-side fairness (C-fairness). According to this definition, XING scenario which was mentioned before, is an example of unfairness for customers. 

The fairness for the item-providers/businesses, who look to hire candidates, means that both local businesses or startups and big corporations, have an equal chance of being exposed/recommended to good candidates. This kind of fairness is called the provider-side fairness (P-fairness). Fairness can be a part of a system goal besides utility, for example in this scenario, if the system tries to match the best job candidates who are a good fit for some companies while trying to meet the fairness needs of either or all the stakeholders. They system can have its own fairness goal as well, such as Kiva Funds\footnote{www.kiva.org}, a micro-lending crown-sourcing non-profit with the mission of providing equal access to capital for any loan-borrower worldwide.

To detect and model bias, several metrics have been introduced for recommendation problems. The metrics presented in \cite{yao2017beyond}, such as absolute unfairness, value unfairness, underestimation and overestimation unfairness focus on the discrepancies between the predicted scores and the true scores across protected and unprotected groups and consider the results to be unfair if the model consistently deviates (overestimates or underestimates) from the true ratings for specific groups. These metrics show unfairness towards customers.

Equality of opportunity discussed in \cite{hardt2016equality} cares about getting equal proportions of individuals from the qualified fractions of each group (equality in true positive rate). This metric can be used both to detect unfairness both for customers and providers.

\cite{celma2008hits} has discussed another type of bias called popularity bias. Many e-commerce websites have this kind of bias such that items from established sellers may dominate recommendation lists because they are more trusted due to having lots of reviews while newly-arrived sellers receive less attention. In this situation, the likelihood of being recommended for popular items will be considerably and unfairly higher than the rest of the items (long-tail items). The methods presented in \cite{abdollahpouri2017controlling, kamishima2014correcting} have tried to break the feedback loop and mitigate this issue. These methods generally try to increase fairness for item providers (P-fairness) in the system by diversifying the recommendation list of users.

There has been some work \cite{eskandanian2017clustering, liu2018personalizing} that try to increase fairness for item-providers by increasing a more diversified set of recommendations to users and some have also offered to consider user’s tolerance for diversity, or in other words users' preferences, to stay fair to customers as well.

The authors in \cite{channamsetty2017recommender} have looked into the influence of algorithms on the output data, but they tracked the extend to which the diversity in user profiles change in the output recommendations. \cite{ekstrand2018exploring} has also looked into the author gender distribution in user profiles in the BookCrossing dataset (BX) and has compared it with that of the output recommendations. According to their results, the nearest neighbor methods propagate the biases and strengthen them and matrix factorization methods strengthen the biases more.

\todo{explain the difference}
Bias disparity paper \cite{tsintzou2018bias}, seeks to demonstrate unfairness for customers/users by modeling the bias as the preferences of users. In this paper we are interested in tracking the change in user preferences (user bias) that recommendation algorithms might have had on the results.

\section{Methodology}
\subsection{Bias Disparity Definition}
Let $\mathcal{U}$ be the set of $n$ users and $\mathcal{I}$ be the set of $m$ items and $S$ be the $n \times m$ input matrix, where $S(u,i) = 1$ if user $u$ has selected item $i$, and zero otherwise. 
 
Let $A_{U}$, be an attribute that is associated with users and partitions them into {\it groups} that have that attribute in common, such as gender. Similarly, let $A_{I}$ be the attribute that is associated with items and that partitions the items into {\it categories} sharing a similar attribute e.g. action or romance genres.
Given matrix $S$, the input {\it preference ratio} for user group G on item category C is the fraction of liked items by group $G$ in category $C$. Formula \eqref{eq:1} is essentially the conditional probability of selecting an item from category C given that this selection is done by a user in group G.
\begin{equation} \label{eq:1}
    PR_{S}(G, C) = \frac{\sum_{u \in G}\sum_{i \in C} S(u, i)}{\sum_{u \in G}\sum_{i \in \mathcal{I}} S(u, i)} 
\end{equation}

Formula \eqref{eq:1} is normalized by $P(C)$, where ${P(C) = {|C|}/{m}}$ is the probability of selecting from category C when we selecting uniformly at random. Then, {\it bias} $B_{S}(G, C)$ for group G on category C is defined as follows:

\begin{equation} \label{eq:2}
    B_{S}(G, C) = \frac{PR_{S} (G, C)}{P(C)}
\end{equation}

Then, {\it positive bias} or bias values greater than 1, happen when a group such as G, on average, tends to like an item category such as C more often. The opposite trend is true for {\it negative bias}.
To compute the bias change in the input $S$ and output of a recommendation algorithm $R$, {\it bias disparity}, that is the relative change of the bias value, is defined as follows:

\begin{equation} \label{eq:3}
    BD(G, C) = \frac{B_{R} (G, C) - B_{S}(G, C) }{B_{S}(G, C)}
\end{equation}

Assuming that a recommendation algorithm provides each user $u$ with a list of $r$ ranked items $R_{u}$, $R$ is the collection of all the recommendations to all the users represented as a binary matrix, where $R(u, i) = 1$ if item $i$ is recommended to user $u$, and zero otherwise.
For more details on this metric, interested readers can refer to \cite{tsintzou2018bias}.

In this paper, we use bias disparity metric on two levels: 1. for different user groups (e.g. women and men) to which we refer as {\it group-based} bias disparity or formula \eqref{eq:3} and \eqref{eq:2}. for all the users in the dataset which we refer to it as {\it general} bias disparity or formula \eqref{eq:4}.

\begin{equation} \label{eq:4}
    BD(C) = \frac{B_{R} (C) - B_{S}(C) }{B_{S}(C)}
\end{equation}
\todo{Do we include formula 4?}

\subsection{Algorithms}
The focus of this research is about the collaborative filtering algorithmic bias. All the recommenders were built via the Librec-auto \cite{mansoury2018automating}, which is a python wrapper built around the core LibRec \cite{guo2015librec} functionality. All the recommenders are built with the 5-fold cross validation setting where 80\% of each user's rating will be considered as the training dataset and the rest as the test dataset (userfixed).

We chose most-popular recommender and random-guess recommender to be our baselines. Theoretically, most-popular recommender generates the recommendation based on the most rated items. So, this algorithm tends to reflect and amplify the popularity bias in the recommendation outputs, which is the key reason we selected this algorithm as our baseline algorithm. Random-guess recommender used in this research, randomly assigns a rating from user $u$ on item $i$. Theoretically, the population of different item categories plays an important role in the bias disparity of a recommender. This provides a different baseline perspective from the most-popular recommender algorithm. 

We chose two commonly used collaborative filtering models for the experiments: neighborhood-based models and latent factor models \cite{koren2009matrix}. We have used both user-based and item-based k nearest neighbor methods in our experiments. From the latent factor models, we selected Biased Matrix Factorization (BiasedMF) \cite{paterek2007improving}, Bayesian Probabilistic Matrix Factorization (BPMF) \cite{salakhutdinov2008bayesian}, and Weighted Regularized Matrix Factorization (WRMF) \cite{hu2008collaborative}, to use in our experiments.m 

\subsection{Datasets}
In our analysis we used two datasets: MovieLens 1M\footnote{https://grouplens.org/datasets/movielens} (ML) and a synthetic dataset.\todo{keep synth. data?}

The first dataset is the MovieLens 1M, a publicly available dataset for movie recommendation which is widely used in Recommender system's domain. ML contains 6,040 users and 3,702 movies and 1M ratings. Sparsity of ratings in this dataset is about 96\%. The second dataset is a synthetic dataset designed for course recommendation and used in \cite{yao2017beyond}. \todo{Nasim: do we have time to do that?}

% \subsubsection{MovieLens 1M}
% The first dataset is the MovieLens 1M, a publicly available dataset for movie recommendation which is widely used in Recommender system's domain. ML contains 6,040 users and 3,702 movies and 1M ratings. Sparsity of ratings in this dataset is about 96\%. 

% We executed two sets of experiments, respectively with Action and Romance movies, and with Crime and Sci-Fi movies. The original ML dataset is filtered based on design of different experiments. The two sets of genres present different prototypes. Both sets have biased input preference but with different sources. The preference bias in the Action and Romance pair comes from the male group, while the female group has a balanced preference over the two genres. The preference bias in the Crime and Sci-Fi comes consistently from both group, which means the preference ratios of the two genres for the two user groups are similar. The comparison of the two experiment sets can present how the bias disparity change for the whole population and sub-groups with different bias sources. \todo{add table describing the characteristics of the two datasets}

% \subsubsection{Synthetic dataset}
% The second dataset is a synthetic dataset designed and used in \cite{yao2017beyond}. This dataset is designed for course recommendation.\todo{do we have time to do that?}

\subsection{Experiment Design}

In this section, we look to address these questions: 
\begin{itemize}
    \item To what extent the preference ratio of men and women is changed by the algorithm in the output?
    \item Is this change limited to a specific group (e.g female users) or does it affect all the users in the dataset?
\end{itemize}

To answer these questions, we take two steps: Initially, we select a subset of the ML dataset consisting of male and female user groups and two movie genres as our item groups. Then, in the {\it first step}, we separately calculate the preference ratio (formula \eqref{eq:1}) of males and females (user groups) on these genres and track their change in the preference ratio using the bias disparity formula (formula \eqref{eq:3}). In the {\it second step}, we calculate the preference ratio on our movie genres on the whole dataset and track the rate of change in this ratio using formula \eqref{eq:4}. 

Generally, if the input preference ratio is significantly different from the output preference ratio in the recommendation, or say the bias disparity is significantly different from 0, it proves the amplification of preference bias.

In the first step of the experiments, we calculate the group-based bias disparity. If the output preference is kept the same as the input preference ratio, it is a fair situation for both groups. Otherwise, it's unfair for the group because their preference is not well presented in the recommendation. If the bias disparity changes to the same degree for both user groups, it shows that although the algorithm reinforces the bias but it is treating both user groups equally. In this scenario, we can not say that it is a fair result for user groups, because their other preferences, however small, are ignored. And if bias disparity change is different for different groups we can draw the conclusion that the algorithm causes disparate impact. 

In the second step of the experiment, we calculate the general bias disparity for the whole population. The comparison of the bias disparity changes for the whole population (step 2) compared to specific user sub-groups (step 1), can help us understand if bias disparity in the data will affect the whole population, ignoring sub-populations or will it affect user groups unevenly.

We executed two sets of experiments, first with Action and Romance genre movies as our item groups, and then with Crime and Sci-Fi genre movies.

\todo{Nicole: add table describing the characteristics of the two datasets}

% We executed two sets of experiments, respectively with Action and Romance movies, and with Crime and Sci-Fi movies. The original ML dataset is filtered based on design of different experiments. The two sets of genres present different prototypes. Both sets have biased input preference but with different sources. The preference bias in the Action and Romance pair comes from the male group, while the female group has a balanced preference over the two genres. The preference bias in the Crime and Sci-Fi comes consistently from both group, which means the preference ratios of the two genres for the two user groups are similar. The comparison of the two experiment sets can present how the bias disparity change for the whole population and sub-groups with different bias sources. \todo{add table describing the characteristics of the two datasets}

% For both experiment sets, the experiment design is similar. First part of the experiment is based on the whole population. Results from this part can present whether the recommendation is with algorithmic bias. If the input preference ratio is significantly different from the output preference ratio in the recommendation, or say the bias disparity is significant different from 0, it proves the existence of algorithmic bias. 

% The second part is based on grouped bias disparity. In this part, the bias disparity is calculated based on the group bias change using the original bias disparity metric in \cite{tsintzou2018bias}, which presents how the bias change of the whole population distributes between groups. If the bias disparity changes to the same degree for different user groups, it shows the algorithm comes with bias but it's fair for different groups. Otherwise, the recommender comes with not only algorithmic bias but also unfairness issue. 

% The fairness discussion can be divided into two levels. The first level is without the consideration of the context. For discussion at this level, it is fair if the values of bias disparity of two groups are similar. Otherwise, the recommendation introduces uneven influence on two user groups, which is defined as unfairness. The second level is about the fairness discussion including context, which is mainly based on the prior condition, the input preference ratio. The input preference ratio presents the initial group preference. If the output preference is kept the same or amplified for the group, it's the fair situation for the group. Otherwise, it's unfair for the group because their preference is not well presented in the recommendation. 
\todo{Nicole:diagram?}

\section{Results}
\subsection{Experiment One: Action and Romance}
In this experiment, we keep the number of items in item groups approximately the same while we create unbalanced user group sizes. The Action and Romance genres are taken as item categories, with 468 and 436 movies in each group respectively. We have 278 women and 981 men for our user groups while each user in these groups has at least 90 ratings. After filtering the dataset, we ended up with 207,002 ratings from 1,259 users on 904 items with a sparsity of 18\% for experiment one. 
As we see in table \ref{ar_input_pref} The preference ratio of male users is higher for Action genre ($\approx0.70$) compared to the Romance genre ($\approx0.30$) whereas female users have a more balanced preference ratio ($\approx0.50$) over these two movie genres. From comparing the preference ratios of the whole population and sub-groups that is shown in Table \ref{ar_input_pref}, there's a overall tendency to like Action genre over Romance genre. This bias can mainly come from the preference ratio of the male user group since we have more men than women. 

\begin{table}[!hbtp]
\centering
\caption{Input Preference Ratio for Action and Romance}
\label{ar_input_pref}
\begin{tabular}{c c c c}
\hline
\textbf{Genre}  & \textbf{Whole Population} & \textbf{Male}  & \textbf{Female} \\ \hline
Action & 0.675 & 0.721 & 0.502 \\ \hline
Romance & 0.325 & 0.279 & 0.498   \\ 
\hline
\end{tabular}
\end{table}

% \subsubsection{Grouped Population}
\subsubsection{Step 1: Group-based Bias Disparity}
For item category Action, the neighborhood methods, UserKNN and ItemKNN, can drive up the preference ratio for both male and female user groups. For different matrix factorization algorithms, the bias change pattern may be different from each other, but all of them are significantly different from the neighborhood methods. With BiasedMF, the preference ratio is lower than the input preference for both groups; with BPMF, the preference ratio of the female group is lower than the input preference ratio, while the male group has a very close preference ratio to the input; with WRMF, the inconsistency is more obvious -- the female group has lower preference ratio and male group is with higher preference ratio. 

For item category Romance, the less favorable item category of the whole population, the phenomenon is similar to the reverse version of Action. For both groups, the neighborhood methods can lower the preference ratio in the recommendation. Different from category Action, the absolute value of the bias disparity for the two user groups are not similar. The male group is with higher absolute value of the bias parity. About the matrix factorization based algorithms, the preference changes are still inconsistent. With BiasedMF, the preference ratio is higher than the input preference ratio for both groups; with BPMF, the female group has a higher preference ratio, while the male group has similar preference ratio as input; with WRMF, the female group has higher preference and male group has lower preference. 

When looking into the fairness issue, the bias disparity over different groups and categories is helpful. It shows how much the recommendation is different from the group's original preference. 

From the first level fairness perspective, ItemKNN introduces more bias to female group than male group in both category Action and Romance, while UserKNN provides more bias to male group than female group in both categories. For BiasedMF, it brings more bias to male group; for BPMF, it brings more bias to female group; for WRMF, the bias disparity shows different direction for male and female groups. When just comparing the absolute value of the bias disparity, for WRMF, it brings more bias to female group than male group. 

From the second level fairness perspective, female group has an almost balanced preference over Action and Romance movies, while male group prefers Action movies to Romance movies. In this case, only balanced preference in the recommendation is fair for female group. However, with the influence of the male group, none of the recommender algorithms provides fairness to the female group. For male group, the neighborhood methods and WRMF amplify the bias and BPMF keep the bias consistent with the input bias, which can be considered as a fair recommendation for male group. Among all the algorithms, BiasedMF is the only one that significantly dampens the bias for male group, which can be considered as a not fair recommendation because it recommends items against the initial preference. 

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_pr_grouped.png}
    \caption{Post Preference Ratio for Action and Romance of Different User Groups}
    \Description{Post preference ratio for the action and romance movie, this is for the grouped population and unbalanced dataset}
    \label{fig:ac_pr_grouped}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_bd_grouped.png}
    \caption{Bias Disparity for Action and Romance of Different User Groups}
    \Description{Bias disparity for the action and romance movie, this is for the grouped population and unbalanced dataset}
    \label{fig:ac_bd_grouped}
\end{figure}

\begin{table}[!hbtp]
\centering
\caption{First Level Fairness for Action and Romance}
\label{ar_first_fairness}
\begin{tabular}{|c|c|}
\hline
\textbf{Algorithm}  & \textbf{More biased group}   \\ \hline
ItemKNN     & Female \\ 
UserKNN     & Male    \\
BiasedMF    & Male  \\ 
BPMF        & Female  \\ 
WRMF        & Male \\
\hline
\end{tabular}
\end{table}

% \subsubsection{Whole Population}
\subsubsection{Step 2: General Bias Disparity}
In Figure \ref{fig:ac_pr_all}, the bar shows the preference ratio in the recommendation output and the dashed line shows the input preference ratio for related categories. 

For Action category, it's the more preferred one between the two categories (0.678). The two neighborhood methods, UserKNN and ItemKNN, both significantly increase the preference ratio. The latent factor model based algorithms, Biased Matrix Factorization (BiasedMF), Bayesian Probabilistic Matrix Factorization (BPMF), and Weighted Regularized Matrix Factorization (WRMF), shows different effect on the preference. None of the matrix factorization algorithms significantly increase the original input preference ratio. For BiasedMF, it significantly decreases the preference ratio in the recommendation, while for BPMF and WRMF, the output preference ratio is very close to the input preference ratio value. 

For Romance category, it has lower input preference ratio, which means in the input dataset, the overall population prefer Action to Romance. As a less favorable category, the preference ratios of Romance show a pattern reverse to the more favorable category, Action. The neighborhood algorithms decrease the preference ratio and the matrix factorization algorithms don't decrease the preference ratio. For biased matrix factorization, it increases the preference ratio, while for the other two matrix factorization algorithms, they don't change the preference ratio very significantly. 

The bias disparity showing in Figure \ref{fig:ac_bd_all} presents the percentage-wise changes of the preference ratio of the two categories over multiple algorithms, which are consistent with the observations from Figure \ref{fig:ac_pr_all}.\todo{extend}

\todo{better viz}
\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_pr_all.png}
    \caption{Post Preference Ratio for Action and Romance}
    \Description{Post preference ratio for the action and romance movie, this is for the whole population and unbalanced dataset}
    \label{fig:ac_pr_all}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/ac_bd_all.png}
    \caption{Bias Disparity for Action and Romance}
    \Description{Bias disparity for the action and romance movie, this is for the whole population and unbalanced dataset}
    \label{fig:ac_bd_all}
\end{figure}

\subsection{Experiment Two: Crime and Sci-Fi}
The other experiment is based on the two genres, Crime and Sci-Fi, respectively with 211 and 276 movies. Users with over 50 ratings of movies from the two genres are selected and are used for the following experiment, resulting 259 female users and 1,335 male users. It turns out to be the experiment dataset including 37,897 ratings from the 1,594 users. 
As it is shown in table (2), the preference bias of both male and female users on Crime and Sci-Fi movies are similar. Both males and females have a preference ratio of around 0.7 on Sci-Fi category and around 0.3 for the Crime genre.
Based on preference shown in Table \ref{cs_input_pref}, the whole population prefer Sci-Fi movies to Crime movies, and for two sub user groups, they have similar preference as the whole population. 

\begin{table}[!hbtp]
\centering
\caption{Input Preference Ratio for Crime and Sci-Fi}
\label{cs_input_pref}
\begin{tabular}{c c c c}
\hline
\textbf{Genre}  & \textbf{Whole Population} & \textbf{Male}  & \textbf{Female} \\ \hline
Crime     &  0.317 & 0.302 & 0.334 \\ \hline
Sci-Fi     & 0.683 & 0.698 & 0.666   \\ \hline
\end{tabular}
\end{table}

% \subsubsection{Grouped Population}
\subsubsection{Step 1: Group-based Bias Disparity}
Overall, the bias disparity of the grouped population patterns is very similar to the whole population pattern. Based on patterns shown in Figure \ref{fig:cs_pr_grouped}, the difference between two groups of same category and algorithm is small. 

From the first level fairness perspective, the difference of bias disparity's absolute value between groups is not as enormous as the difference shown in Action and Romance (Figure \ref{fig:ac_bd_grouped}), which is partly because the two groups have similar preference over the two experimented categories. 

From the second level fairness perspective, neighborhood based algorithms can amplify the existing preference bias for both groups. The matrix factorization based algorithms either dampen the input preference ratio, like BiasedMF and BPMF, or don't significantly change the input preference, like WRMF. 

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_pr_grouped.png}
    \caption{Post Preference Ratio for Crime and Sci-Fi of Different User Groups}
    \Description{Post preference ratio for the Crime and Sci-Fi, this is for the grouped population and unbalanced dataset}
    \label{fig:cs_pr_grouped}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_bd_grouped.png}
    \caption{Bias Disparity for Crime and Sci-Fi of Different User Groups}
    \Description{Bias disparity for the Crime and Sci-Fi movie, this is for the grouped population and unbalanced dataset}
    \label{fig:cs_bd_grouped}
\end{figure}

\begin{table}[!hbtp]
\centering
\caption{First Level Fairness for Crime and Sci-Fi}
\label{ar_first_fairness}
\begin{tabular}{|c|c|}
\hline
\textbf{Algorithm}  & \vline \textbf{More biased group}   \\ \hline
ItemKNN     & Female \\ 
UserKNN     & Female    \\ 
BiasedMF    & Male \\ 
BPMF        & Male  \\ 
WRMF        & Male(f=10) and Female(f=20)  \\ 
\hline
\end{tabular}
\end{table}

% \subsubsection{Whole Population}
\subsubsection{Step 2: General Bias Disparity}
As shown in the Figure \ref{fig:cs_pr_all}, the pattern of Crime and Sci-Fi over the whole population is consistent with Action and Romance. The neighborhood based algorithms, UserKNN and ItemKNN, increase the preference of category with the higher input preference, meanwhile decrease the preference of less favorable category. The matrix factorization based algorithms show different patterns from neighborhood based algorithms but very similar pattern as it's shown in the experiments with Action and Romance. For BiasedMF, it has the most significant effects on preference, which increase the preference of less favorable category and decrease the preference of the more favorable category. For BPMF and WRMF, the preference change is not that obvious. 

The bias disparity showing in Figure \ref{fig:cs_bd_all} presents the percentage-wise changes, which is also consistent with the bias disparity shown in the Figure \ref{fig:ac_pr_all} of experiment one.

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_pr_all.png}
    \caption{Post Preference Ratio for Crime and Sci-Fi}
    \Description{Post preference ratio for the Crime and Sci-Fi movie, this is for the whole population and unbalanced dataset}
    \label{fig:cs_pr_all}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots/cs_bd_all.png}
    \caption{Bias Disparity for Crime and Sci-Fi}
    \Description{Bias disparity for the Crime and Sci-Fi movie, this is for the whole population and unbalanced dataset}
    \label{fig:cs_bd_all}
\end{figure}

\section{Discussion}
According to our results, When there’s an existing general bias in the data, some of the recommendation algorithms, such as K nearest neighbor method, amplify these biases whereas matrix factorization algorithms either perpetuate or dampen the bias. As we have discovered in our experiments, recommendation algorithms don’t explicitly benefit or harm specific user groups (in our case men and women) or item groups (genres), but they pick up a bias in the data that might be in favor or against a group and change them.
\todo{to extend}

\section{Conclusion and Future Work}
Different kinds of biases might exist in the real world and they can be reflected in the training data and picked up, modeled and amplified by recommendation algorithms. This process can create and strengthen the filter bubbles wherein we live and can reinforce the stereotypes that can potentially lead to disparate impact. Applying machine learning algorithms blindly on the data, runs the risk of amplifying biases present in data. So we need to initially detect these biases and eventually control their influence by de-biasing the data, or mitigating their influence in the training process of the model or output results.
\todo{extend}


==> body_v3.tex <==
\section{Introduction}
Recommender systems have become ubiquitous and are increasingly influencing our daily decisions in a variety of online domains. Recently, there has been a shift of focus from achieving the best accuracy \cite{herlocker2004evaluating} in recommendation to non-accuracy measures such as diversity, novelty and to more socially-sensitive concerns such as fairness \cite{hurley2011novelty, jannach2015recommenders}. One of the key issues with which to contend is that biases in the input data (used for training predictive models) are reflected, and in some cases amplified, in the results of recommender system algorithms. This specially important in contexts where fairness and equity matters and/or is required by law such as in lending (Equal Credit Opportunity Act), education (Civil Rights Act of 1964; Education Amendments of 1972), housing (Fair Housing Act), employment (Civil Rights Act of 1964), etc.

% \cite{mehrotra2018towards}
% \todo{example from spotify?}

The biases in the outputs of recommendation algorithms can be due to a variety of factors in the input data that is fed to the algorithm. As the saying goes: “garbage in, garbage out”. These underlying factors include \cite{barocas2016big} sample size disparity, having limited features for protected groups, features that are proxies of demographic attributes, human factors or skewed findings. These causes are not mutually exclusive and can be present at the same time and they can result in disparate negative outcomes. 

In this paper, we model \textit{bias} as the preferences of users and their tendency to choose an item over the other. In and of itself, this type of bias is not necessarily a negative phenomenon. In fact, patterns in preference bias is the key ingredient of  recommendation algorithms to construct predictive models and provide users with personalized outputs. However, in certain contexts the propagation of preference biases can be problematic. For example, in the news recommendation domain, preference biases can cause filter bubbles \cite{pariser2011filter} and limit the exposure of users to diversified items. And, in job recommendation and lending domains, existing biases in the input data may reflect historical societal biases against protected groups which must be accounted for by learning systems.

Our main goal in this paper is to study how different collaborative filtering algorithms might propagate or amplify existing preference bias in the input data and the different kinds of impact bias disparity between the input and the output of such algorithms might have on users.
%In recent recommender systems research, a number of metrics for measuring unfairness have been introduced. 
For the purpose of this analysis, we use \textit{bias disparity}, a recently introduced group-based metric\cite{tsintzou2018bias,zhao2017men}. This metric considers biases with respect to the preferences of specific user groups such as men or women towards specific item categories such as different movie genres. This metric evaluates and compares the preference ratio in both the input and the output data and measures the degree to which recommendation algorithms may propagate these biases, in some cases weakening them and in others amplifying them. Throughout this paper we use the notions of preference bias and preference ratio interchangeably.

%Different classes of recommendation algorithms have various logic behind them and thus have different behaviors. These different behaviors can change the bias of the output data differently. We analyze and compare the extent to which common collaborative filtering algorithms can change the existing biases. 

Our preliminary experiments on a movie rating dataset show that different types of algorithms behave quite differently in the way in which they propagate preference biases in the input data. These findings maybe especially important for system designers in determining the choice of algorithms and parameter settings in critical domains where the output of the system must conform to legal and ethical standards or to prevent discriminatory behavior by the system. As far as we know, this paper is among the first works to have observed this phenomenon in recommendation algorithms. 
%This analysis helps developers and researchers to beware of the discriminatory properties of CF algorithms and to think of removing the issues before designing a system.

We are specifically interested in answering the following research questions: 
\begin{itemize}
    \item \textbf{RQ1} How do different recommendation algorithms propagate existing preference biases in the input data to the generated recommendation lists?
    \item \textbf{RQ2} How does the bias disparity between the input and the output differ for different user groups (e.g., men versus women)?
   % \item \textbf{RQ3} How does bias change on an individual level for users with extremely positive or extremely negative preferences towards an item category?
    \item \textbf{RQ3} How do bias disparity effects impact individual users with extreme preferences (positive or negative) with respect to particular categories?
\end{itemize}

%\textbf{Roadmap}: In section 2 we briefly introduce the previous related research upon which we base our work. In section 3 (Methodology), we define the notion of {\it bias disparity} and how to calculate it. We also discuss the design of our experiments, the algorithms and the dataset that we have used in this paper. The results of our experiments, the discussion of those results, and our conclusions are presented in sections 4, 5 and 6, respectively.
% RB: This is not necessary in a paper that is this short.

\section{Related work}

As authors in \cite{burke2018balanced} mention, fairness can be a multi-sided notion. Recommender system often involve multiple stakeholders, including consumers and providers \cite{burke2016towards} and fairness can be sought for for these different stakeholders. In general, fairness is a system goal, as neither side have a good view of the ecosystem and distribution of the resources. Fairness for users/consumers could mean providing similar recommendations to similar users without considering their protected attributes, such as certain demographic features. Methods that seek fairness for consumers of a system fall under the category of consumer-side fairness (C-fairness). Fairness to item-providers (for example sellers on Amazon), may means providing their items a reasonable chance of being exposed/recommended to consumers. This kind of fairness is called the provider-side fairness (P-fairness).
% As an example of unfairness for consumers, take XING\footnote{www.xing.com}, a job platform similar to LinkedIn, which was found to rank less qualified male candidates higher than more qualified female candidates \cite{lahoti2019ifair}.


Various metrics have been introduced for detecting model biases. The metrics presented in \cite{yao2017beyond}, such as absolute unfairness, value unfairness, underestimation and overestimation unfairness focus on the discrepancies between the predicted scores and the true scores across protected and unprotected groups and consider the results to be unfair if the model consistently deviates (overestimates or underestimates) from the true ratings for specific groups. These metrics show unfairness towards consumers.

Equality of opportunity discussed in \cite{hardt2016equality} detects whether there are equal proportions of individuals from the qualified fractions of each group (equality in true positive rate). This metric can be used to detect unfairness for both consumers and providers.
Steck \cite{steck2018calibrated} has proposed an approach for calibrating recommender systems to reflect the various interests of users relative to their initial preference proportions.
% \todo[inline]{The work of Steck  on calibration really needs to be mentioned here. See steck2018calibrated in the bibliography.}


The authors in \cite{celma2008hits} have discussed another type of bias called popularity bias. Many e-commerce websites have this kind of bias such that items from established sellers may dominate recommendation lists because they are more trusted due to having lots of reviews while newly-arrived sellers receive less attention. In this situation, the likelihood of being recommended for popular items will be considerably and unfairly higher than the rest of the items (long-tail items). The methods presented in \cite{abdollahpouri2017controlling, kamishima2014correcting} have tried to break the feedback loop and mitigate this issue. These methods generally try to increase fairness for item providers (P-fairness) in the system by diversifying the recommendation list of users.

%There has been some work \cite{eskandanian2017clustering, liu2018personalizing} that try to increase fairness by providing a more diversified set of recommendations to users and some have also offered to consider user’s tolerance for diversity, or in other words users' preferences, to stay fair to consumers as well.
% RB: Diversity takes us far afield from the topic of this paper

The authors in \cite{channamsetty2017recommender} have looked into the influence of algorithms on the output data; they tracked the extent to which the diversity in user profiles change in the output recommendations. \cite{ekstrand2018exploring} has also looked into the author gender distribution in user profiles in the BookCrossing dataset (BX) and has compared it with that of the output recommendations. According to their results, the nearest neighbor methods propagate the biases and strengthen them and matrix factorization methods strengthen the biases more. Interestingly, our results for matrix factorization methods show the opposite trends possibly indicating the different behavior of algorithms in different domains and datasets.

The work by Tsintzou et al. \cite{tsintzou2018bias} sought to demonstrate unfairness for consumers/users by modeling the bias as the preferences of users. They analyze the result only for K-nearest-neighbor models. In this paper, we build on their work by considering a variety of recommendation algorithms. We are also interested in understanding bias changes affect different user groups and how they might affect individual users.


\section{Methodology}

\subsection{Bias Disparity}

Let $\mathcal{U}$ be the set of $n$ users and $\mathcal{I}$ be the set of $m$ items and $S$ be the $n \times m$ input matrix, where $S(u,i) = 1$ if user $u$ has selected item $i$, and zero otherwise. 
 
Let $A_{U}$, be an attribute that is associated with users and partitions them into {\it groups} that have that attribute in common, such as gender. Similarly, let $A_{I}$ be the attribute that is associated with items and that partitions the items into {\it categories} sharing a similar attribute e.g. movie genres.

Given matrix $S$, the input {\it preference ratio} for user group $G$ on item category $C$ is the fraction of liked items by group $G$ in category $C$. Formula \eqref{eq:1} is essentially the conditional probability of selecting an item from category C given that this selection is done by a user in group G.
\begin{equation} \label{eq:1}
    PR_{S}(G, C) = \frac{\sum_{u \in G}\sum_{i \in C} S(u, i)}{\sum_{u \in G}\sum_{i \in \mathcal{I}} S(u, i)} 
\end{equation}

Then, {\it bias} $B_{S}(G, C)$ for group $G$ on category $C$ is defined as follows:

\begin{equation} \label{eq:2}
    B_{S}(G, C) = \frac{PR_{S} (G, C)}{P(C)},
\end{equation}

Where ${P(C) = {|C|}/{m}}$ is the probability of selecting an item uniformly at random from category $C$. To make formula \eqref{eq:2} comparable across different item categories, formula \eqref{eq:1} is normalized by $P(C)$. The higher the bias, the higher (on average) the tendency of a group such as $G$, to like a category such as $C$.

To compute the bias change between the input $S$ and output of a recommendation algorithm $R$, {\it bias disparity}, that is the relative change of the bias value, is defined as follows:

\begin{equation} \label{eq:3}
    BD(G, C) = \frac{B_{R} (G, C) - B_{S}(G, C) }{B_{S}(G, C)}
\end{equation}

Assuming that a recommendation algorithm provides each user $u$ with a list of $r$ ranked items $R_{u}$, $R$ is the collection of all the recommendations to all the users represented as a binary matrix, where $R(u, i) = 1$ if item $i$ is recommended to user $u$, and zero otherwise. For more details on this metric, interested readers can refer to \cite{tsintzou2018bias}.

In this paper, we use bias disparity metric on two levels: 1. For different user groups of women and men, to which we refer to as {\it group-based} bias disparity or formula \eqref{eq:3}. 2. For all the users in the dataset to which we refer to as {\it general} bias disparity or formula \eqref{eq:4} which is defined below:

\begin{equation} \label{eq:4}
    BD(C) = \frac{B_{R} (C) - B_{S}(C) }{B_{S}(C)}
\end{equation}

A bias disparity of near zero, means that the input preference bias of a user or a group of users hasn't been changed in the output. If the bias disparity value is greater than 0, we have a {\it positive} bias disparity. In this case, the output preference bias towards an item category is higher than that of the input. In other words, the preference bias is reinforced or amplified by the algorithm. As an example, if women like Romance genre more, now in their recommendation list they see Romance movies disproportionately to their actual preferences. A {\it negative} bias disparity means that the output preference bias is greater than that of the input. In other words, the preference bias is reversed. As an example, if men like Action genre, now they see disproportionately less of that genre in their recommendation lists.

\subsection{Algorithms}

All the recommendation algorithms were built via the Librec-auto \cite{mansoury2018automating}, which is a python wrapper built around LibRec \cite{guo2015librec}, a Java library for recommendation algorithms. In our experiments, we built the recommenders with a 5-fold cross validation setting where 80\% of each user's rating data is considered for the training dataset and the rest as the test dataset (userfixed).

We tested our experiments on four groups of algorithms: memory-based, ranking, rating and baseline. We chose most-popular recommender to be one of our baselines. We selected both user-based and item-based k-nearest-neighbor methods from the memory-based category. BPR \cite{rendle2009bpr}, RankALS \cite{takacs2012alternating} were selected from the learning-to-rank category. From the latent factor models (rating algorithms) \cite{koren2009matrix}, we selected Biased Matrix Factorization (BiasedMF) \cite{paterek2007improving}, SVD++ \cite{koren2008factorization}, and Weighted Regularized Matrix Factorization (WRMF) \cite{hu2008collaborative}. Theoretically, most-popular recommender generates the recommendation based on the most rated items. This algorithm tends to amplify the popularity bias in the recommendation outputs, which is the key reason we selected this algorithm as our baseline algorithm.
For each algorithm, we tuned the parameters and picked the one that gives the best performance in terms of normalized discounted cumulative gain (NDCG) of the top 10 listed items, precision and recall. The NDCG of the algorithms over two experiments in the paper is shown in Table \ref{tab:NDCG}. 
% The highest NDCG value comes from BPR algorithm in both experiments. Meanwhile, BiasedMF and SVD++ have the lowest NDCGs among all the algorithms. 

\begin{table}[!hbtp]
\centering
\begin{tabular}{c | c c c}
\hline
\textbf{Algorithm}  & \textbf{Experiment 1} & \textbf{Experiment 2} \\ \hline
MostPopular & 0.480 & 0.460 \\ \hline
ItemKNN & 0.524 & 0.515 \\ \hline
UserKNN & 0.572 &  0.559 \\ \hline
BPR & \hl{\textbf{0.616}} & \hl{\textbf{0.588}} \\ \hline
RankALS & 0.446 & 0.374 \\ \hline
BiasedMF & 0.200 & 0.200 \\ \hline
SVD++ & 0.167 &  0.239\\ \hline
WRMF & 0.507 & 0.498 \\ \hline
\end{tabular}
\caption{NDCG values with selected parameters for the two experiments}
\label{tab:NDCG}
\end{table}

\subsection{Dataset}

We ran our experiments on MovieLens 1M\footnote{https://grouplens.org/datasets/movielens} dataset (ML), a publicly available dataset for movie recommendation which is widely used in Recommender system's domain. ML contains 6,040 users and 3,702 movies and 1M ratings. Sparsity of ratings in this dataset is about 96\%.

\subsection{Experiment Design}

In this section, we look to address these questions: 
\begin{itemize}
    \item To what extent the preference ratio of men and women is changed by a CF algorithm in the output? (RQ2)
    \item Is this change limited to a specific group (e.g female users) or does it affect all the users in the dataset? (RQ1)
    \item For users with extreme initial preference ratio, what's the effect on the preference ratio from different algorithms? (RQ3) 
\end{itemize}
% \todo{complete}

We addressed these questions in three steps: Initially, we selected a subset of the ML dataset consisting of male and female user groups and two movie genres as our item groups. Then, in the {\it first step}, we separately calculated preference ratio (formula \eqref{eq:1}) of males and females (user groups) on these genres and tracked their change in the preference ratio using the bias disparity formula (formula \eqref{eq:3}). In the {\it second step}, we calculated the preference ratios for our movie genres on the whole user data (without partitioning into separate user groups) and tracked the rate of change in this ratio using formula \eqref{eq:4}. In the {\it third step}, we looked into users with zero initial preference ratio on one of the genres to see the effects of BD on them. Our goal was to determine if input preference ratios were significantly different from the output preference ratios in the recommendations (i.e., if bias disparity was significantly different from 0, resulting in the amplification of preference biases either negatively or positively). 

In the first step of the experiments, we calculated the group-based bias disparity. If the output preference is kept the same as the input preference ratio, we consider it a fair situation for both groups. Otherwise, the recommendations may represent unfairness for the group because their preferences is not well represented in the recommendation lists. If the bias disparity changes to the same degree for both user groups, it shows that although the algorithm reinforces the bias, it is still treating both user groups equally. In this scenario, we can not say that it is a fair result for user groups, because their other preferences, however small, are ignored. And if bias disparity change is different for different groups we can draw the conclusion that the algorithm causes disparate impact. Whether this different treatment leads to unfairness would depend on the specific domain.

In the second step of the experiment, we calculated the general bias disparity for the whole population. The comparison of the bias disparity changes for the whole population (step 2) compared to specific user sub-groups (step 1), can help us understand if bias disparity in the data will affect the whole population, ignoring sub-populations or will it affect user groups unevenly.

We ran two sets of experiments, first with Action and Romance genre movies as our item groups, and then with Crime and Sci-Fi genre movies. More details will be mentioned in each experiment.

\section{Experimental Results}

\subsection{Experiment One: Action and Romance}

In this experiment, we keep the number of items in item groups approximately the same while we create unbalanced user group sizes. The Action and Romance genres are taken as item categories, with 468 and 436 movies in each group respectively. We have 278 women and 981 men for our user groups while each user has at least 90 ratings. After filtering the dataset, we ended up with 207,002 ratings from 1,259 users on 904 items with a sparsity of 18\% for experiment one. 

As we see in Table \ref{tab:ar_input_pref}, the preference ratio of male users is higher for Action genre ($\approx0.70$) compared to the Romance genre ($\approx0.30$) whereas female users have a more balanced preference ratio ($\approx0.50$) over these two movie genres. From comparing the preference ratios of the whole population and sub-groups (table \ref{tab:ar_input_pref}), we observe an overall tendency to like Action genre over Romance genre. This overall bias can mainly come from the preference ratio of the male user group since we have more men than women. 
% Then the recommendation algorithm tends to recommend the preference of the majority group more to all the users, ignoring the preference of the minority groups.

\begin{table}[!hbtp]
\centering
\begin{tabular}{c c c c}
\hline
\textbf{Genre}  & \textbf{Whole Population} & \textbf{Male}  & \textbf{Female} \\ \hline
Action & 0.675 & 0.721 & 0.502 \\ \hline
Romance & 0.325 & 0.279 & 0.498   \\ 
\hline
\end{tabular}
\caption{Input preference ratio for Action and Romance}
\label{tab:ar_input_pref}
\end{table}

\subsubsection{Step 1: Group-based Bias Disparity}
% knn
According to the results shown in Figure \ref{fig:ac_pr}, we see that both the neighborhood based methods, UserKNN and ItemKNN, increased the preference ratio (PR) of both male and female user groups on Action genre by 50\% and around 20\% respectively. While both of these algorithms have increased the PR on Action genre, they have dramatically decreased it for Romance genre, although the PR of women on both genres were balanced. As we see in Figure \ref{fig:ac_bd}, both of these algorithms show negative bias disparities (BD) on Romance for both men and women. These results suggest that the neighborhood-based methods tend to perpetuate and amplify the existing biases in the input data (further moving the generated recommendations towards Action movies and away from Romance movies). 

% mf
On the other hand, matrix factorization algorithms show a different tendency. 

In BiasedMF, the output preference ratio is much lower than the input preference ratio for male users in the Action genre (the opposite of what we observed for the neighborhood-based methods). The PR for the female group is approximately the same. With BiasedMF, the PRs of both female and male groups are pushed close to 0.5. We have a negative bias disparity as we see in Figure \ref{fig:ac_bd}, which means that the original preference ratio is underestimated. Interestingly, this algorithm strengthens the bias disparity of both men and women on Romance genre which is an overestimation of their actual preference. We see a similar pattern in SVD++ as well.

%In BPMF, the input and output preference ratio for both Action and Romance genres and for both user groups of men and women is approximately the same. So, this algorithm keeps the PR almost the same.

WRMF, the other latent factor model, gives inconsistent results from BiasedMF and SVD++. It slightly decreased the PR of women on Action and increased the PR of men on Action. We see the opposite trend on Romance genre, in other words, the output PR for women on Romance is slightly higher while for men is lower. 

Generally, the absolute value of the BD for the two user groups are not similar. Men have higher absolute values of BD on Romance while women have higher absolute values of BD on Action. As we see in Figure \ref{fig:ac_bd}, different algorithms affect women or men differently. ItemKNN affects the women more than men in both genres, while UserKNN amplifies the bias more for men than women in both genres. BiasedMF and SVD++ increase bias more for men; WRMF, increases the bias slightly more for women.

In this experiment, women had an almost balanced preference over Action and Romance movies, while men prefer Action movies to Romance movies. In this case, according to the recommendation calibration definition, a balanced preference ratio in the recommendation output is expected. However, with the influence of the male group, most of the recommender algorithms provide an unbalanced recommendation list specially for women(the minority group). Although, BiasedMF and SVD++ reverse the bias disparity for both genres. So the influence of men's preferences for Action in the overall data is reduced resulting in fewer unwanted Action movie recommendations for women which is more fair for this group. These two algorithms balance out the exposure of Action and Romance genres for both user groups.

% [SOME ADJUSTEMENT NEEDED HERE] For men, the BPMF keeps the bias almost consistent with the input bias, which can be considered fair, according to Table \ref{ar_first_fairness}. In this algorithm, still the bias disparity is slightly more for women. 

% The neighborhood based methods and WRMF amplify the bias which is unfair since it ignores every aspect of this user group. Among all these algorithms, BiasedMF and SVD++ significantly decreases the bias for men, which is unfair because it recommends items against the initial preference. 


% can be used for conclusion
K-nearest-neighbor methods amplify the bias significantly and this behavior could be due to their sensitivity to the popularity bias.
% Both of the neighborhood-based models show a similar trend to the most-popular recommender (the light blue bar). Romance genre is less favored by the majority group (981 men vs 278 women) in the dataset compared to the Action genre. So, we end up having more neighbors from the majority group as the nearest neighbors (user-knn) or having more ratings from the majority group on a specific genre (item-knn). So, their preference will dominate the preference of the other group on both genres. These methods not only prioritize the preference of the majority group to the minority group, but they also amplify this bias in a way that it changes the original PR of the majority group itself.

\begin{table}[!hbtp]
\centering
\begin{tabular}{|c|c|c|c|}%So, do we need 
\hline
\textbf{Algorithm}  & \textbf{Women} & \textbf{Men}   \\ 
\hline
MostPopular & \textbf{2.519} & 0.659 \\ 
ItemKNN     & \textbf{2.100} & 0.994\\ 
UserKNN     & 0.749 & \textbf{1.091}\\
BPR         & 0.285 & \textbf{0.678}\\
RankALS     & \textbf{0.368}  & 0.306\\
BiasedMF    & 1.230  & \textbf{2.660}\\ 
SVD++       & 0.803  & \textbf{2.364}\\ 
WRMF        & \textbf{0.585}  & 0.523\\
\hline
\end{tabular}
\caption{Bias disparity absolute value sum over Action and Romance}
\label{ar_first_fairness}
\end{table}



\subsubsection{Step 2: General Bias Disparity}

In Figure \ref{fig:ac_pr}, the bar shows the preference ratio in the recommendation output and the dashed line shows the input preference ratio for related categories. 

The Action genre (PR as 0.675) is preferred to the Romance genre (PR as 0.325). The two neighborhood-based methods, UserKNN and ItemKNN, both increase the general preference ratio significantly. While our latent factor models: BiasedMF, SVD++, WRMF, show different effects on the preference ratio. None of the matrix factorization algorithms significantly increase the original input preference ratio in the Action genre. BiasedMF and SVD++ significantly decreases the output preference ratio in Action genre, while WRMF keep the the output preference ratio close to the initial preference. 

The Romance category has lower input preference ratio than Action genre, which means that in the input dataset, the population on average prefer Action to Romance. The output preference ratios for this genre show a reverse pattern compared to the Action genre. The neighborhood-based algorithms decrease the preference ratio and most of the matrix factorization algorithms don't change the preference ratio by much except for BiasedMF and SVD++, which significantly increases the preference ratio. We can see the bias disparity change in Figure \ref{fig:ac_bd} as well.

% The bias disparity showing in Figure \ref{fig:ac_bd_all} presents the percentage-wise changes of the preference ratio of the two categories over multiple algorithms, which are consistent with the observations from Figure \ref{fig:ac_pr_all}.\todo{extend}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots_v3/ar_pr_1.png}
    \caption{Output Preference Ratio for Action and Romance}
    \Description{Post preference ratio for the action and romance movie, this is for the whole population and the subgroup populations in unbalanced dataset}
    \label{fig:ac_pr}
\end{figure}

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots_v3/ar_bd_1.png}
    \caption{Bias disparity for Action and Romance}
    \Description{Bias disparity for the action and romance movie, this is for the whole population and the subgroup populations in unbalanced dataset}
    \label{fig:ac_bd}
\end{figure}

\subsubsection{Step 3: Users with Extreme Preferences}

% In both experiments, there is a small user group with initial preference ratio of zero on one category or both. It means these users watched all the movies only from one genre or haven't watched from both genres. These users were excluded from the bias disparity calculations.
We excluded the users that had a zero PR on both genres. in the dataset, we had 10 men who had zero PR on the Romance genre, which means that they only watched Action movies. In Figure \ref{fig:ac_eg}, it shows the preference ratio in the recommendation. Some algorithms, like UserKNN, BPR, and WRMF, recommend all Action movies, which is totally consistent with these users initial preference. Algorithms, including BiasedMF and SVD++, de-amplify the effects on the preference. When analyzing the preference ratio of the extreme group, the effects of some algorithms become more clearer because of the consistency of the general population and extreme group. 

% In this experiment, there are only 10 users with zero input preference ratio. All of them are male users who only watched Action movies. 
% When analyzing the preference ratio of the extreme group, the effects of some algorithms become more clearer because of the consistency of the general population and extreme group. 
% Different matrix factorization methods behave differently in this case. 
% BPR and WRMF, recommendations are closer to the user's initial preferences, while for BiasedMF and SVD++, the recommendations result in decreasing the preference ratios among users. 

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots_v3/ar_extremegroup.png}
    \Description{Post preference ratio for the action and romance movie, this is for the whole population and the subgroup populations in unbalanced dataset of the extreme group}
    \caption{Output PR for users with extreme preferences for Action and Romance}
    \label{fig:ac_eg}
\end{figure}

\subsection{Experiment Two: Crime and Sci-Fi}

In this experiment our item groups were Crime and Sci-Fi, with 211 and 276 movies in each group respectively. The number of users in both user groups were still unbalanced, 259 female users and 1,335 male users. All of the users had at least 50 ratings from both genres which leaves us with 37,897 ratings from the 1,594 users on 487 item. The sparsity of the dataset was around 5\%.

As it is shown in table \ref{tab:cs_input_pref}, the preference ratios of both male and female users in Crime and Sci-Fi movies are similar. Both men and women have a preference ratio of around 0.7 on Sci-Fi and around 0.3 for the Crime genre. According to table \ref{tab:cs_input_pref}, the whole population prefers Sci-Fi movies to Crime movies, and we see a similar trend in both user groups, male and female. 

\begin{table}[!hbtp]
\centering
\begin{tabular}{c c c c}
\hline
\textbf{Genre}  & \textbf{Whole Population} & \textbf{Male}  & \textbf{Female} \\ \hline
Crime     &  0.317 & 0.302 & 0.334 \\ \hline
Sci-Fi     & 0.683 & 0.698 & 0.666   \\ \hline
\end{tabular}
\caption{Input Preference Ratio for Crime and Sci-Fi}
\label{tab:cs_input_pref}
\end{table}

\subsubsection{Step 1: Group-Based Bias Disparity}

Overall, the group-based bias disparity is very similar to the pattern that we see for the whole population. Based on patterns shown in Figure \ref{fig:cs_pr}, the difference between the patterns that we see in Crime genre for both men and women is minimal. the same trend is true for Romance genre.
The difference in the absolute values of bias disparity between groups is not as enormous as the difference that we saw in Action and Romance (Figure \ref{fig:ac_bd}), which is partly because the two groups have similar preference over the two categories. 

Neighborhood-based algorithms amplify the existing preference bias for both groups. The matrix factorization algorithms either dampen the input bias, like BiasedMF and SVD++, or they don't change the input preference ratio significantly, like WRMF. 

\begin{table}[!hbtp]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Algorithm}  & \textbf{Women} & \textbf{Men}   \\ \hline
MostPopular & 0.740 & \textbf{0.951} \\ 
ItemKNN     & \textbf{1.137} & 0.898\\ 
UserKNN     & \textbf{0.818} & 0.792\\
BPR         & 0.357 & \textbf{0.400}\\
RankALS     & \textbf{1.126} & 1.114\\
WRMF        & 0.247  & \textbf{0.311}\\
BiasedMF    & 3.089  & \textbf{3.636}\\ 
SVD++       & 2.394  & \textbf{2.778}\\ 
\hline
\end{tabular}
\caption{Bias disparity absolute value sum over Crime and Sci-Fi}
\label{ar_first_fairness2}
\end{table}

\subsubsection{Step 2: General Bias Disparity}

As shown in the Figure \ref{fig:cs_pr}, the pattern of Crime and Sci-Fi over the whole population is consistent with Action and Romance. The neighborhood based algorithms, UserKNN and ItemKNN, increase the output preference ratio for the more preferred genre (Sci-Fi), meanwhile they decrease the preference ratio for the less preferred genre (Crime). The matrix factorization algorithms show different patterns from neighborhood based algorithms but very similar pattern to experiment 1. BiasedMF and SVD++ has the most significant effects on the preference ratio. It increases the PR of the less favorable category and decrease the PR of the more favorable category. WRMF, the PR change is not obvious. 

The bias disparity showing in Figure \ref{fig:cs_bd} is also consistent with the bias disparity shown in the Figure \ref{fig:ac_bd} of experiment one.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots_v3/cs_pr_1.png}
    \caption{Output preference ratio for Crime and Sci-Fi}
    \Description{Output preference ratio for the Crime and Sci-Fi movie, this is for the whole population and subgroup populations in unbalanced dataset}
    \label{fig:cs_pr}
\end{figure}

% [!hbtp]
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots_v3/cs_bd_1.png}
    \caption{Bias disparity for Crime and Sci-Fi}
    \Description{Bias disparity for the Crime and Sci-Fi movie, this is for the whole population and subgroup populations in unbalanced dataset}
    \label{fig:cs_bd}
\end{figure}
% \todo[inline]{I would recommend separating out the ``learning to rank'' algorithms from the others by color. These are BPR and RankALS. Then you wouldn't be trying to distinguish five shades of blue.}

\subsubsection{Step 3: Users with Extreme Preferences} 

We had 37 users with PR value of zero on Crime movies, meaning that they only watched Sci-Fi movies. The trends that we see in Figure \ref{fig:cs_eg} for this group is pretty similar to Figure \ref{fig:ac_eg}

% In the Crime and Sci-Fi comparison, the size of the extreme group is 38 with 5 female users and 33 male users. In this extreme group, 37 out of 38 users only watched Sci-Fi movies, and one user only watched Crime movies.

% In this part discussion, only the group watching all Sci-Fi movies are taken into discussion. 
% In , the Sci-Fi only extreme group shows similar pattern as the Action and Romance genres in .
Similarly to experiment one, algorithms such as UserKNN, BPR, and WRMF, provide the recommendations with the exact same PR as users' initial preferences whereas BiasedMF and SVD++, significantly de-amplify the initial preference ratios. 

% limitation and future work: one limitation is that the size of the extreme group is small. Diving into individual level bias disparity of this kind of extreme group is interesting but needs more individuals for valid conclusion. 

\begin{figure}[!hbtp]
    \centering
    \includegraphics[width=\linewidth]{plots_v3/cs_extremegroup.png}
    \caption{Output Preference Ratio for Crime and Sci-Fi of Extreme Group}
    \Description{Post preference ratio for the crime and sci-fi movie, this is for the whole population and the subgroup populations in unbalanced dataset of the extreme group}
    \label{fig:cs_eg}
\end{figure}

% \section{Discussion}

\section{Conclusion and Future Work}

Both of the neighborhood-based models show a similar trend to the most-popular recommender. Romance genre is less favored by the majority group (981 men vs 278 women) in the dataset compared to the Action genre. So, we end up having more neighbors from the majority group as the nearest neighbors (user-knn) or having more ratings from the majority group on a specific genre (item-knn). So, their preference will dominate the preference of the other group on both genres. These methods not only prioritize the preference of the majority group to the minority group, but they also amplify this bias in a way that it changes the original PR of the majority group itself.

% both whole population and subgroups (two gender groups) over both genres in both of our experiments which is a different conclusion from . 

% Different from SVD++ and BiasedMF, WRMF algorithm preserve the whole population bias in both experiments. However, when the initial preference ratio of subgroups different from the whole population, like women group in experiment one, the preference of the subgroup can't be preserved. However, for groups with more similar initial PR to the whole population, the preference could be more preserved, like the male group in experiment one, and both female and male groups in experiment two. 

Different from the previous research on the bias amplification of matrix factorization methods \cite{ekstrand2018exploring}, we observed that different matrix factorization models show different results and influence the bias differently. So, there is no general conclusion on these algorithms. SVD++ and BiasedMF both balance out the preference bias on different movie genres for both men and women. WRMF algorithm preserves the PR for the Sci-Fi/Crime pair for both men and women but the behavior is inconsistent for Action/Romance genre. We repeated a similar experiment on BPMF, and observed that it preserves the PR for men and women for all genres.

This results could be because these algorithms provide a low rank representation for users and items and this dimensionality reduction could remove some of the noise/bias in the input data and help balance out the results. Interestingly, parameter tuning of these algorithms although resulted in better accuracy but it didn't change the bias disparity pattern.

As we have discovered in our experiments, recommendation algorithms pick up an existing bias in the data that might be in favor or against a group and change them, sometimes in unexpected ways. Thus the choice of recommendation algorithm is critical in the design of a recommender system, particularly when there are strong existing biases in the preference data. Applying machine learning algorithms blindly on the data, runs the risk of amplifying biases present in data. So we need to initially detect these biases and eventually control their influence in the training process of the model or the output results.

The real reason behind the differences in the output of of these algorithms needs further analysis and will be investigated in the future. Whether these differences in the results of these algorithms are due to their vulnerability to popularity bias or not, needs further exploration. It would be interesting to see if the same effects will happen in other data sets. We are also interested to investigate the influence of users with extreme preferences on the general results of the recommendations.
